MEGAN: Multi-Explanation Graph Attention Network

We propose a multi-explanation graph attention network (MEGAN). Unlike existing graph explainability methods, our network can produce node and edge attributional explanations along multiple channels, the number of which is independent of task specifications. This proves crucial to improve the interpretability of graph regression predictions, as explanations can be split into positive and negative evidence w.r.t to a reference value. Additionally, our attention-based network is fully differentiable and explanations can actively be trained in an explanation-supervised manner. We first validate our model on a synthetic graph regression dataset with known ground-truth explanations. Our network outperforms existing baseline explainability methods for the single- as well as the multi-explanation case, achieving near-perfect explanation accuracy during explanation supervision. Finally, we demonstrate our model's capabilities on multiple real-world datasets. We find that our model produces sparse high-fidelity explanations consistent with human intuition about those tasks.

==> sections/__04_experiments.tex <==
\section{Computational Experiments}
\label{sec:experiments}

%
% FIGURE: RbMotifs Examples
% -------------------------------
%
\begin{figure*}[h!]
\begin{center}
%\includegraphics[width=1.0\textwidth]{figures/rbmotifs_new.pdf}
\end{center}
\caption{Examples for explanations generated for one element of the RbMotifs dataset using selected methods. We point out that in this instance GNNExplainer fails to discover the second relevant explanatory motif. Even though GNES and single-channel MEGAN correctly highlight both motifs, the single-channel explanations fail to capture the fact that both motifs represent \textit{opposing} evidence. Only the multi-channel methods correctly capture the polarity of influence for both motifs, increasing the interpretability of the explanations.}
\label{fig:rbmotifs-all}
\end{figure*}
%

In this section, we only give a brief overview of the used datasets and experiments. Details about the datasets can be found in Appendix~\ref{app:datasets}. Details on hyperparameters and empirical results for experiments are listed in Appendix~\ref{app:experiments}

%%%%%%%%%%%%
% DATASETS %
%%%%%%%%%%%%

\subsection{Datasets}

\textbf{RbMotifs.  } We create a synthetic graph regression dataset consisting of 5000 randomly generated graphs, where each node has three node features representing an RGB color value. Edges are undirected and unweighted. Some of these randomly generated colored graphs are additionally seeded with specific subgraph motifs, which consist of pre-defined color combinations and are associated with a constant value. When a motif appears in a graph, the associated value is added to that graph's overall value.

\textbf{Solubility.  } Approx. 8000 molecular graphs of the AqSolDB dataset \cite{sorkun_aqsoldb_2019}. The target value for each graph is the value of the measured log representing the water solubility of the corresponding chemical compound. Node and edge features are generated by RDKit \cite{landrum_rdkit_2010}.

\textbf{MovieReviews.  } A dataset of 2000 movie reviews, classified by sentiments "positive" and "negative". Originally a text-based dataset from the ERASER benchmark \cite{deyoung_eraser_2020}, we pre-processed it into a graph dataset by
representing each word as a node and connecting adjacent nodes by undirected and unweighted edges using a sliding window of size 2.

\textbf{TADF Singlet-Triplet Energy Splittings.  } Approx. 500000 molecular graphs of the TADF dataset \cite{gomez-bombarelli_design_2016}. We use the singlet-triplet energy splittings $\Delta E_{\text{ST}}$ as the target value, which is one of two primary parameters to assess thermally activated delayed fluorescence (TADF) properties of molecules. Molecules with such TADF character are promising candidates for novel, low-cost OLED materials \cite{endo_efficient_2011, zhang_design_2012}.

%%%%%%%%%%%
% METRICS %
%%%%%%%%%%%

% -- TABLE: RB MOTIFS COMPARISON
% \input{tables/rbmotifs_all}

\subsection{Metrics} 
\label{sec:metrics}
\label{sec:fidelity}

We measure similarity to the ground truth explanations using AUROC, as it is done by \cite{mccloskey_using_2019}. We measure sparsity on binarized explanations, which are generated by thresholding the model's continuous attributions. We also measure explanation fidelity as described in \cite{yuan_explainability_2022} and additionally provide the fidelity of random explanations for comparison. More details can be found in Appendix~\ref{app:experiments-metrics}.

For the multi-explanation models, we define the $\text{Fidelity}^{*}$ metric: Considering regression as an example, we argue that the positive explanation channel is faithful to the predicted output, exactly if the model output becomes significantly more \textit{negative} when the positive channel is withheld from the model, as it is then missing all supposedly positive information about the graph. The same applies to the negative channel, which when withheld, should produce a more positive output. In this sense, we calculate a deviation $\Delta y^{k}$ for each channel by supplying a corresponding binary importance mask $\mathbf{M}^{k}$ (see Figure \ref{fig:architecture}) which completely blocks channel $k$. A channel's deviation then contributes positively to the overall value if that deviation is along the expected direction as defined before:
\begin{equation}
    \text{Fidelity*} = \frac{1}{K} \sum_{k=1}^K \begin{cases}
        +\Delta y^k & \text{if deviation as expected} \\
        -\Delta y^k & \text{if deviation \textit{not} as expected } \\
    \end{cases}
\end{equation}
Consequently, positive values of $\text{Fidelity*}$ show good alignment of explanations with their respective channel's intended interpretation, while low and negative values indicate misalignment.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SINGLE CHANNEL EXPERIMENTS %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Synthetic Dataset - Single Explanations}

% VERSION 1 - BEFORE REVIEWS
% The reviews wanted more baseline experiments, which is what I did and thus this entire section had to be rewritten

% We demonstrate the base capabilities of our model for the special single-explanation ($K = 1$) case. The experiment is conducted on the synthetic RbMotifs graph regression dataset. We compare explanations of a baseline $\text{MEGAN}^{K=1}_{\gamma = 0.0}$ model, an explanation-supervised $\text{MEGAN}^{K=1, \text{(S)}}_{\gamma = 0.0}$ model and the explanations of GNNExplainer based on a simple GCN network with similar layer structure.\\
% The experiment is repeated independently 50 times, where a new random dataset split is chosen each time. We report our results in Table~\ref{tab:rbmotifs-all} and show examples in Figure~\ref{fig:rbmotifs-all}.

% The results show that both MEGAN models greatly outperform the GCN baseline in terms of the main predictions (MSE, $\text{R}^2$). The baseline $\text{MEGAN}^{1}_{0.0}$ and GNNExplainer perform comparably in terms of similarity to ground truth, while the explanation-supervised $\text{MEGAN}^{1}_{0.0}$ clearly outperforms both, nearly achieving a perfect match. We also point out, that explanations of MEGAN models show noticeably larger median fidelity than the random baseline, while explanations of GNNExplainer don't, indicating that explanations produced by MEGAN actually faithfully reflect the model's predictive behavior.\\

% Generally, in the single-explanation case, we often observe that with samples where the graph contains two opposing motifs (red and blue) the explanations of baseline $\text{MEGAN}^{1}_{0.0}$ and GNNExplainer usually focus only on either of the motifs, as it can be seen in Figure~\ref{fig:rbmotifs-all}(a). Only the explanation-supervised $\text{MEGAN}^{1, \text{(S)}}_{0.0}$ correctly highlights both motifs.

% VERSION 2 - NOVEMBER 2022
We demonstrate the capabilities of our model first for the basic single-channel explanation ($K = 1$) case. The experiment is conducted on the synthetic RbMotifs dataset. We primarily compare regression performance (MSE, $\text{r}^2$) and similarity to know ground truth explanations (Node AUC, Edge AUC). We compare with established post-hoc baselines Grad, GradCAM \cite{pope_explainability_2019} and GNNExplainer \cite{ying_gnnexplainer_2019}. Additionally, we compare with the explanation supervision method GNES \cite{gao_gnes_2021}, which we had to modify to facilitate proper applicability to regression problems (details in Appendix~\ref{app:gnes}). We report our results in Table~\ref{tab:rbmotifs-all} and illustrate examples in Figure~\ref{fig:rbmotifs}.
\\
Our results show that the explanation-supervised single-channel version $\text{MEGAN}_{0.0}^{1, \text{(S)}}$ of our network outperforms the runner-up modified GNES model by a significant margin, achieving almost perfect node and edge explanation accuracy. Additionally, our model also significantly outperforms the GCN models used as the basis for the other methods in terms of predictive performance.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MULTIPLE CHANNEL EXPERIMENTS %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Synthetic Dataset - Multi Explanations}
%
% FIGURE: SOLUBILITY MAIN
% -----------------------
%
\begin{figure*}[h!]
\centering
%\includegraphics[width=1.0\textwidth]{figures/solubility_main.pdf}
\vspace*{-0.4cm}
\caption{Selected examples of explanations for the prediction of solubility. top: dual-channel explanations generated by MEGAN, bottom: single-channel explanations generated by GnnExplainer. Darker highlights for nodes and edges indicate higher predicted importance values. }
\label{fig:solubility_main}
\end{figure*}

% VERSION 1 - BEFORE REVIEWS
% The reviews wanted more baseline experiments, which is what I did and thus this entire section had to be rewritten
% In the second experiment, we demonstrate our model's capability to learn dual explanations ($K = 2$). %
% The experiment is conducted on the synthetic RbMotifs graph regression dataset. We compare multiple architecturally identical  $\text{MEGAN}^K_{\gamma}$ models and vary the value of the explanation training hyperparameter $\gamma$, including a baseline model with $\gamma = 0$, which performs no additional explanation training step at all, and an explanation-supervised version $\text{MEGAN}^{2,\text{(S)}}_{0.0}$\\
% Each experiment is independently repeated 50 times, where a new random dataset split is chosen each time. We report our results in Table~\ref{tab:rbmotifs-all} and show an example in Figure~\ref{fig:rbmotifs-all}.

% The results show that the baseline $\text{MEGAN}^{2}_{0.0}$ model achieves the lowest similarity to the ground truth explanations, with $\text{MEGAN}^{2,\text{(S)}}_{0.0}$ showing the highest value, achieving a near perfect match for nodes and edges. For the prediction performance on the other hand there is no clear difference between the models, all of them achieving nearly identical $\text{R}^2$ values. The  $\text{Fidelity}^{*}$ is also the highest for the explanation-supervised model $\text{MEGAN}^{2,\text{(S)}}_{0.0}$, while the models with $\gamma \neq 0$ result in similarly high median values, although the distributions show higher deviation for lower values of $\gamma$. The baseline model $\text{MEGAN}^2_{0.0}$ shows the lowest median $\text{Fidelity}^{*}$ value with the highest  fluctuations. 

% We first conclude that explanation supervision can be applied effectively to train a MEGAN model to emulate pre-defined explanations. Secondly, the proposed modified training procedure also leads to the development of explanations that have high similarity to ground truth and are faithful to the intended channel interpretations when compared to the baseline. In this context, it is also important to note that the baseline model $\text{MEGAN}^2_{0.0}$ does not perform significantly differently on the prediction task. In fact, we generally observe that this model learns the correct explanations as well, but without any additional guidance, the alignment of these explanations with the two available channels is arbitrary. This often leads the correct explanations to develop in the wrong channels (w.r.t their intended interpretation) as can be seen in Figure~\ref{fig:rbmotifs-all}.

% VERSION 2 - NOVEMBER 2022
In the second experiment, we demonstrate our model's capability when moving to multi-channel explanations ($K = 2$). In this case, the existing ground truth explanations were also split into two channels, where the first channel contains all those explanatory motifs that contribute negatively to a graph's label and the second channel contains all those motifs that contribute positively. Our results firstly show that the regression performance of our model is further increased when employing an additional channel. Additionally, the explanation supervised version $\text{MEGAN}^{2, \text{(S)}}_{0.00}$ is able to correctly learn explanations, even as they are split into different channels, as indicated by the near perfect explanation accuracy. More importantly, $\text{MEGAN}^2_{1.00}$ which is not explanation-supervised but uses the explanation co-procedure achieves similarly good results.

We illustrate the added value of multi-channel explanations in the example in Figure~\ref{fig:rbmotifs}. We argue that the multi-channel explanations add a highly valuable dimension to the interpretability of explanations: While some of the single-channel are able to identify the explanatory motifs accurately, the singular explanations fail to capture that in reality both of the motifs represent semantically \textit{opposing} evidence. The multi-channel MEGAN model however is able to correctly decipher this property of the motifs, even without external intervention in the form of explanation supervision. Moreover, during our experiments, we notice that single-channel methods often fail to identify two motifs of opposing evidence in the same graph and we assume that this fact is a major reason for the bad performance of the baseline methods for datasets of this type.

%%%%%%%%%%%%%%%%%%%%%%%
% REAL WORLD DATASETS %
%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Real-World Datasets}

Besides the synthetic dataset, we also apply our model on several real-world datasets. We report hyperparameters for these experiments and the detailed results in Appendix~\ref{app:real_experiments}.

% DISCUSSION OF MOVIE REVIEWS RESULTS
% -------------------------------------

The MovieReviews dataset requires the binary classification of movie review sentiment into the two classes "negative" and "positive". In terms of classification, our model performs comparably to baseline GNN approaches from literature, yet significantly worse than state-of-the-art NLP approaches (Table~\ref{tab:movie_results}). However, we find that our model still produces explanations consistent with human intuition, as it appropriately declares negative adjectives like "bad", "unfunny" and "disappointing" as explanations for the negative class and likewise positive adjectives like "good", "remarkable" and "clever" as explanations for the positive class. We illustrate one example movie review along with our model's explanations in Table~\ref{tab:movie-reviews} and more in Appendix~\ref{app:examples-movie-reviews}.

% 
% TABLE: MOVIE REVIEWS EXAMPLE
% ----------------------------
%
%\input{tables/movie_reviews}

% DISCUSSION OF SOLUBILITY RESULTS
% --------------------------------

The Solubility dataset requires the prediction of the logS value for water solubility of various chemical compounds. For this task, we a truncated comparison of results in Table~\ref{tab:solubility_short}. Our model is able to achieve regression performance, similar to results from the literature and other state-of-the-art GNNs. The results also show that our model consistently produces explanations which are sparse and faithful to the predicted value.
Figure \ref{fig:solubility_main} shows examples of explanations produced by our model, as well as single-channel explanations produced by GnnExplainer. We find that explanations of our model accurately reproduce chemical intuition about this task. Large non-polar carbon structures are consistently provided as explanations for negative influence, while polar oxygen and nitrogen functional groups are highlighted as positive influence on the target value. We argue that, in comparison, the single-channel explanations generated by GnnExplainer are considerably less interpretable for humans.

% DISCUSSION OF TADF RESULTS
% --------------------------

% VERSION 1 - 01.11.2022
% ----------------------
% This is from the final ICLR version of the paper

% We also apply our model to the prediction of the singlet-triplet energy gap from the TADF dataset. Our model achieves a high predictivity of $r^2 = 0.9$ on the regression task. Additionally, the explanations of our model are able to reproduce non-trivial structure-property relationships from chemical knowledge. As shown in Figure~\ref{fig:tadf}(a) for example, triphenylamine bridges are known to be associated with low energy gaps, as they cause the necessary twist angles between the fragments, decoupling electron donating and
% electron accepting parts of a molecule to reduce the exchange interaction between the frontier orbitals
% which would otherwise lower the triplet state compared to the singlet state, thus preventing undesired
% singlet-triplet splittings. We are also able to support hypotheses published in previous work by \cite{friederich_scientific_2021}, who use an interpretable decision tree method to generate explanatory hypotheses for the same task. Our model for example also finds conjugated bridges as positive evidence and carbonyl groups as negative evidence as shown in Figure~\ref{fig:tadf}(b). Furthermore, we are able to propose novel hypotheses for explanatory motifs: As shown in Figure~\ref{fig:tadf}(c), we for example observe silane groups and phosphine oxides to be consistently highlighted as evidence for high target values. In total, we propose 5 new motifs as shown in Appendix~\ref{app:examples-tadf}.

% VERSION 2 - 22.01.2023
% ----------------------
% For the ICLM version of the paper we decided to switch the focus from the TADF results back to the solubility results since that should be easier to understand for laymen, requiring this section to be significantly shortened.

We also apply our model to the prediction of the singlet-triplet energy gap from the TADF dataset. Our model achieves high regression predictivity of $R^2 = 0.9$, comparable to results from the original publication \cite{gomez-bombarelli_design_2016}. Additionally, the sparse high-fidelity explanations generated by our model are able to reproduce non-trivial structure-property relationships from chemical knowledge, such as triphenylamine bridges being associated with low energy splittings. We can support hypotheses of explanatory sub-graph motifs proposed by earlier work \cite{friederich_scientific_2021} and are able to propose 5 novel explanatory motifs based on the MEGAN's explanations. Details can be found in Apendix~\ref{app:tadf}.

%
% TABLE: SOLUBILITY RESULTS
% -------------------------
%
%\input{tables/solubility_results_short.tex}

%%%%%%%%%%%%%%%%%%%%%%%%
% BENCHMARKING RESULTS %
%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{GNN Benchmarks}

Aside from explainability experiments, we also test our model on standard GNN benchmarks. Selected benchmarking results for the two popular graph regression datasets ESOL and Lipop are shown in Table \ref{tab:benchmark_short}. More detailed information can be found in Appendix \ref{app:benchmarks}. We find that MEGAN is able to match the predictive performance of state-of-the-art GNNs, achieving the second-best result for both datasets. This indicates that good performance and explainability don't necessarily have to be a trade-off. Moreover, this indicates that the inherent explanation mechanism might even improve performance.
%
%\input{tables/benchmarks_short.tex}

